A Toolkit for Generating Code Knowledge Graphs

Knowledge graphs have been proven extremely useful in powering diverse applications in semantic search and natural language understanding. In this paper, we present GraphGen4Code, a toolkit to build code knowledge graphs that can similarly power various applications such as program search, code understanding, bug detection, and code automation. GraphGen4Code uses generic techniques to capture code semantics with the key nodes in the graph representing classes, functions, and methods. Edges indicate function usage (e.g., how data flows through function calls, as derived from program analysis of real code), and documentation about functions (e.g., code documentation, usage documentation, or forum discussions such as StackOverflow). Our toolkit uses named graphs in RDF to model graphs per program, or can output graphs as JSON. We show the scalability of the toolkit by applying it to 1.3 million Python files drawn from GitHub, 2,300 Python modules, and 47 million forum posts. This results in an integrated code graph with over 2 billion triples. We make the toolkit to build such graphs as well as the sample extraction of the 2 billion triples graph publicly available to the community for use.

==> sections/conclusions.tex <==
\section{Conclusions}

We presented Graph4Code, a toolkit capable of building code knowledge graphs that connect code analysis with other diverse sources of knowledge about code such as documentation and user-generated content in forum posts. 
To demonstrate the effectiveness and scalability of this toolkit, we applied it over 1.3 million Python programs and 47 million forum posts to generate a code knowledge graph of over 2 billion triples. We also show the  promise of such a knowledge graph with 1) a set of SPARQL templates to help users query the graph, and 2) an assessment of the coverage and precision of the links it generates.  With this toolkit, we hope to mimic the success and widespread applications of general knowledge graphs, but in the code understanding domain. Therefore, we hope that {\logo}  will help the community build better code representations, and consequently better tools for code automation, code search and bug detection.

==> sections/cross_validate_paths.tex <==
\subsection{Code suggestion}
Another use of the knowledge graph could be to provide code suggestions for data scientists.  To evaluate the potential to use the knowledge graph for this use case, we evaluated how many data flow edge successors existed for path lengths of 1, 2, and 3 in test programs.  A path length of 1 assumes only one turtle call site had been written in the code, where a data scientist had made one API call to a data science library, and the question is how well we could predict the very next set of calls using the knowledge graph.  Similarly, path lengths of 2 and 3 model the case when the data scientist has written two or three API calls, and the question being asked is how many suggestions on average we would predict using the knowledge graph.  We note that this is a relatively naive way to use the knowledge graph for code completion, but we do so to evaluate the quality of the graph for the use case rather than suggesting that a code completion system be designed in this way. As before, we evaluated this using a 10 fold split of test programs, where we rotated each set as the `test' case, and used the remaining nine sets to model the knowledge graph we could query against.  

\begin{figure}
\centering 
{\includegraphics[width=0.4\textwidth]{path_length_1}}%
\hfill 
{\includegraphics[width=0.4\textwidth]{path_length_2}}%
\hfill 
{\includegraphics[width=0.4\textwidth]{path_length_3}}%
\caption{Path lengths of 1, 2 and 3}
\label{cross_validate_paths}
\end{figure}

Figure~\ref{cross_validate_paths} shows the percentage of paths in the test programs of length 1, 2 and 3 we found in the knowledge graph across the 10 splits.  As shown in the figure, when we were able to find 97.5\% of paths of length 1 in the knowledge graph, 88.9\% of paths of length 2, and 68.9\% of paths of length 3.  Of those, 71.1\% of paths of length 1 had successors, 57.1\% of paths of length 2 had successors, and 39.5\% of paths of length 3 had successors.  Figure~\ref{cross_validate_means} shows the average number of successors for different path lengths across the 10 runs.  The average number of successors across runs was 176.5 for paths of length 1, 49.9 for paths of length 2, 7.3 for paths of length 3. 

\begin{figure}
\centering  
{\includegraphics[width=0.45\textwidth]{sublime}}
\caption{Code suggestions in Sublime Text 3}
\label{code_suggestion_ide}
\end{figure}
  
While there are many enhancements that could improve an actual code suggestion system---e.g., considering control flow edges to prune successors, analyzing if objects exist that could flow into parameters that are needed for successors, etc., these results suggest that with sufficient context (i.e., more API calls written by the user to infer intent), the knowledge graph can actually be used provide a small enough number of successors as suggestions.  To make this concrete, in Figure~\ref{code_suggestion_ide}, we show a screenshot of prototype code suggestions in Sublime Text 3 based on our knowledge graph.  The user hovers over the {\tt PCA.decomposition.sklearn} constructor, and the tool runs the SPARQL query in Figure~\ref{code:code_suggestion_sparql} on our knowledge graph after substituting {\tt PCA.decomposition.sklearn} for {\tt ?m}.   The query suggests {\tt fit} variants as something to do next, as that is what our graph shows is most common.

\begin{figure}[htb]
\begin{centering}
\lstinputlisting[language=Python,escapechar=|]{./code_suggestion_sparql.txt}
\caption{SPARQL query for code suggestions}
\label{code:code_suggestion_sparql}
\end{centering}
\end{figure}

\begin{figure}
\centering 
{\includegraphics[width=0.5\textwidth]{avg_successors}}
\caption{Path lengths of 1, 2 and 3}
\label{cross_validate_means}
\end{figure}



==> sections/dataset.tex <==
\subsection{Dataset}

We used Google's BigQuery public GitHub dataset of over 3 million open source projects\footnote{\url{https://console.cloud.google.com/marketplace/details/github/github-repos?filter=solution-type:dataset&q=github&id=46ee22ab-2ca4-4750-81a7-3ee0f0150dcb}} to extract Python files or Python notebooks that import SciKit Learn\footnote{Note that SciKit Learn is one of the more popular data science libraries, and as we showed in the turtles we included, this does tend to include many other popular data science libraries such as SciPy, TensorFlow, etc.}.  This query yielded 9489 files. Of these, we kept only the files that could be parsed by a Python 3 or Python 2 parser.  Duplicate files were eliminated, with duplicates defined as files with the same MD5 hashcode.  This yielded 6671 files, 6474 files of which could be successfully analyzed by our framework for a 97.04\% success rate. Most files were analyzed within a second, with a few taking a few minutes.


==> sections/graph.tex <==
\subsection{Knowledge Graph}
\label{sec:graph}

To make the analysis IR useful for multiple purposes, we created a knowledge graph from it.  We describe the graph construction in this section and then present uses for the graph in subsequent sections.  Unlike previous work that stores analysis information in a database, our knowledge graph aims to enable convenient queries about the relationships among APIs and their usage.  The graph for the running example from Figure~\ref{running_example} is shown in Figure~\ref{fig:rdf_graph}; it explicitly represents data flow as black arrows in the picture and control flow as orange arrows, with edge labels denoting the kind of flow.

 To see how the edges are generated, consider the IR in Figure~\ref{code:ann_post}.  Instruction 2 is a call to the function read from the {\tt read\_csv} field of the {\tt pandas} object read from {\tt pd}, denoted as node 104 in Figure~\ref{fig:rdf_graph}.  Since the {\tt read\_csv} field is considered the same as {\tt pandas} by the analysis, {\tt pandas} itself is considered the receiver of the call, hence the receiver edge from node 10.  Similarly the {\tt constant\_arg} edge denotes the file name argument of the read call.  Then instructions 6-8 call the {\tt to\_list} function on the turtle it generates, so it becomes the receiver for that call, which is denoted by node 105.  To make this knowledge graph easy to query for multiple use cases, we adopted the W3C standard of RDF (Resource Description Framework)\footnote{\url{https://www.w3.org/RDF/}}, so we could easily issue declarative queries using the associated SPARQL\footnote{\url{https://www.w3.org/TR/sparql11-query/}} query language to query the knowledge graph. 

\begin{figure*}[htb]
\begin{center}
\includegraphics[width=5in]{rdf_fig}
\end{center}
\caption{RDF representation of turtles in running example}
\label{fig:rdf_graph}
\end{figure*}


==> sections/linking.tex <==



\subsection{Data Linking}


% Central to all the different components is the documentation strings 
Figure~\ref{fig:schema} shows the schema of {\logo}. Node and edges in code analysis are created through the static analysis of Python programs. \textit{Software execution} nodes correspond to method calls which are also linked to their input and output nodes via \textit{sio:has\_input} and \textit{sio:has\_output} edges. Whevener possible, these nodes are also linked via an \textit{rdf:type} edge to their corresponding type; i.e., method, function or class. In docstrings, each function, method or class is associated with its documentation via \textit{skos:definition},  \textit{skos:notation}, \textit{rdfs:label} ... etc. Class heirarichy information is also maintained via \textit{dct:isPartOf} links. 

To link the forum posts, we relied on the ElasticSearch index built for StackOverflow and StackExchange. For each class, function or method in docstrings, we performed elastic search query to get all the relevant forum posts. The relevant posts are then added to the graph with all its details; e.g. title, question, list of answers, votes, codes .. etc. We then use a \textit{schema:about} edge to connect each forum post to its corresponding class, function or method. 


% The central component that links the different data sources together is the documentation of  
% To connect all the data sources together, we used docstrings as the center piece of the graph. In particular, all other module connect to docstrings by referring to the same method, function or class name used in docstrings. Figure~\ref{fig:schema} gives an overview of the schema of graph4code. At the heart of the graph lies the information extracted from docstrings which captures the heirarchy of the function or class with documentations extracted 



% \subsection{Linking Documentation Data to Code Static Analysis}

% The basic static analysis graph has XXX triples; out of which there is around 6M triples that are candidates for linking to other documentation from various sources. Some of these entities can be resolved to functions and classes. However, it also contains plain module names, function arguments such as constant and dictionaries, python common functions and constructors such as \textbf{hasattr, type, super}. These nodes can not be linked to any any other data source; hence they are excluded. This results in only 2M entities that we can extend. 

% For each object in these triples, we tried to resolve it to see if it matches a function or a class. For example, \textit{re.compile} is a direct match to the function \textit{compile} in python module \textit{re}. Similarly \textbf{tensorflow.Session.run} maps directly to the function \textit{Session.run} in \textit{tensorflow} while \textit{os.path} is a direct class match. However, this is not always the case, sometimes resolving these entities is not very straightforward. Objects such as \textit{matplotlib.pyplot.figure.add_subplot.plot} and \textit{argparse.ArgumentParser.add_subparsers.add_parser.set_defaults} are typically hard to resolve since classes and function names  .... 

% One a match is found, the corresponding graph node is extended with links to the matched documentation from docstrings, documentation usage and Stackoverflow. This resulted in an additional XXX triples added to the base static analysis graph. 




\subsection{Linking Documentation and Forum Discussions to Usage}
\label{sec:linking}
To link the usage data to the code documentation, the user documentation and the Stack Overflow discussions, we started from the paths we observe in the code from program analysis.  Note that if a user code contains the following line of code:
\begin{verbatim}
pandas.read_csv("foo").merge(x).merge(y)
\end{verbatim}
the entities associated with the return values of the four expressions will have turtle paths reflecting the succession of accesses:
\begin{enumerate}
\item {\tt{pandas.read\_csv.merge.merge}} 
\item {\tt{pandas.read\_csv.merge}}
\item {\tt{pandas.read\_csv}}
\item {\tt{pandas}}
\end{enumerate}
The last two represent the initial import of {\tt pandas} and the call to {\tt read\_csv}, both of which can be linked directly to their associated documentation.  Those are our direct matches.  However, for the {\tt merge} calls, there are no formal types that tells us what {\tt read\_csv} returns.  While docstrings do sometimes provide return types, it is often in an informal manner: e.g. read\_csv is said to return a {\tt DataFrame}, but with nothing to qualify that to a specific module.  Interpreting this documentation when possible is future work. For now, we adopted the strategy of mapping it to the longest prefix we could find in the documentation and StackOverflow.  As long as a prefix matched, those are our partial matches.  If no prefix matched we call it a missed link.  

\begin{figure}[htb]
\begin{center}
\includegraphics[width=.85\linewidth]{paper_figures/Linking.pdf}
\end{center}
\caption{Linking static analysis results to documentation}
\label{fig:link_analysis_docs}
\end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=.75\linewidth]{paper_figures/LinkingDocstrings.pdf}
\end{center}
\caption{Linking docstrings to StackOverflow and usage docs}
\label{fig:docstring_link_analysis_docs}
\end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=.75\linewidth]{paper_figures/LinkingDocstringsInspect.pdf}
\end{center}
\caption{Linking docstrings-inspect to StackOverflow and usage docs}
\label{fig:docstring_link_analysis_docs_inspect}
\end{figure}

It is important to note that we modeled every import in code as a `library' which often includes user code.  We are therefore not likely to find a high percentage of links back to library code that is used very heavily across users. The unique number of path objects in the static analysis graph is 2,024,443.  Figure \ref{fig:link_analysis_docs} shows the number of unique methods, classes, and functions we found across data sources.  Not surprisingly, the best coverage came from docstrings; in some cases, the docstrings from AST and docstrings from inspect on live Python modules.  There may be some duplication with results from the two sources; however, they represent names in non-uniform and different styles, making this hard to assess rigorously.  Fixing this requires further linking work in the future.

Figure \ref{fig:docstring_link_analysis_docs} shows the linkages we found from docstrings to StackOverflow and to the usage documentation.  For docstrings, the overall number of classes was 253,590, methods was 275,903, and functions was 1,165,402.  As shown in the figure, we did better in linking to StackOverflow documents than to usage documentation, which is not very surprising because usage documentation is usually targeted at specific classes.  No function mentions occurred in usage documentation either, which is again not too surprising because the documentation tends to be focused on classes and how they can be used.  

Figure \ref{fig:docstring_link_analysis_docs_inspect} shows linkages we found from docstrings-inspect to StackOverflow and to usage documentation.  For docstrings gleaned from inspection, the overall number of classes was 83,408, the overall number of functions was 103,448 and number of methods was 2,118,990.  The trend was similar to the docstrings data, with lower linking numbers.




==> sections/static_analysis_linking.tex <==
\subsection{Linking Documentation Data to Code Static Analysis}

The basic static analysis graph has XXX triples; out of which there is around 6M triples that are candidates for linking to other documentation from various sources. Some of these entities can be resolved to functions and classes. However, it also contains plain module names, function arguments such as constant and dictionaries, python common functions and constructors such as \textbf{hasattr, type, super}. These nodes can not be linked to any any other data source; hence they are excluded. This results in only 2M entities that we can extend. 

For each object in these triples, we tried to resolve it to see if it matches a function or a class. For example, \textit{re.compile} is a direct match to the function \textit{compile} in python module \textit{re}. Similarly \textbf{tensorflow.Session.run} maps directly to the function \textit{Session.run} in \textit{tensorflow} while \textit{os.path} is a direct class match. However, this is not always the case, sometimes resolving these entities is not very straightforward. Objects such as \textit{matplotlib.pyplot.figure.add_subplot.plot} and \textit{argparse.ArgumentParser.add_subparsers.add_parser.set_defaults} are typically hard to resolve since classes and function names  .... 

One a match is found, the corresponding graph node is extended with links to the matched documentation from docstrings, documentation usage and Stackoverflow. This resulted in an additional XXX triples added to the base static analysis graph. 

==> sections/uses.tex <==
\subsubsection{Code Assistance: Next Coding Step}

\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{paper_figures/next_step.png}
\end{center}
\caption{Finding most commonly used next step}
\label{fig:next_step}
\end{figure}


% \begin{figure*}[h!]
% \scriptsize
% \centering
% \begin{verbatim}
%         select (count(?g) as ?c) ?predict ?prev_type where {
%          graph ?g {
%           ?prev        a           py:sklearn.ensemble.RandomForestClassifier .
%             #  ?prev ('has input'/^'has output')+ ?equiv.
%           ?prev        sio:SIO_000229/^sio:SIO_000230  ?equiv .
%           ?equiv       a       py:sklearn.ensemble.RandomForestClassifier.predict .
%           ?equiv       sio:SIO_000229/^sio:SIO_000230  ?next .
%           ?next        a       ?predict .
%           filter( ?predict != prov:Activity
%             #      && ?classifierName != 'software execution'
%                 && ?predict != sio:SIO_000667
%                 && ?predict != py:print
%                 && ?predict != graph4code:Function)
%             }
%         } group by ?predict ?prev_type order by desc(?c) limit 3
% \end{verbatim}
% \caption{Query to find the next step in a program}
% \label{fig:next_step_query}
% \end{figure*}

\begin{figure*}[h!]
% \scriptsize
\centering
\begin{verbatim}
select (count(?g) as ?c) ?next_label where {
    graph ?g {
         ?pred      rdfs:label          "sklearn.ensemble.RandomForestClassifier" .
         ?pred      graph4code:flowsTo+ ?this .
         ?this rdfs:label               "sklearn.ensemble.RandomForestClassifier.predict" .
         ?this rdf:type                 <http://semanticscience.org/resource/SIO_000667> .
         ?this graph4code:flowsTo+      ?next .
         ?next rdfs:label               ?next_label .
         ?next rdf:type                 <http://semanticscience.org/resource/SIO_000667> .
    }
} group by ?next_label order by desc(?c) limit 3
\end{verbatim}
\caption{Query to find the next step in a program}
\label{fig:next_step_query}
\end{figure*}


In this use case, we integrated {\logo} inside and IDE and used it for code assistance to find the most commonly used next steps, based on the context of their own code. Context, in this query, means data flow predecessors of the node of interest; in this case, we take a simple example of the single predecessor call that constructed the classifier.  Figure~\ref{fig:next_step} shows an example of a real Kaggle notebook, where users can select any expression in the code and get a list of the most common next steps along with the frequency with which the next step is observed.  For example, in similar contexts after a \texttt{model.predict} call, data scientists typically do one of the following: 1) build a text report showing the main classification metrics (frequency: 16), 2) report  the confusion matrix which is an important step to understand the classification errors (frequency: 10) and 3) save the prediction array as text (frequency: 8). This can help users by alerting them to best practices from other data scientists.  In the example shown above, the suggested step of adding code to compute a confusion matrix is actually useful.  The existing Kaggle notebook does not contain this call, but the call is very helpful to understand the properties of a classifier. 

We show in Figure~\ref{fig:next_step_query} the SPARQL query used to support this use case. 
The query variable \textit{?this} is the node that has an execution path of ``sklearn.ensemble.RandomForestClassifier.predict`` where the user is at in the program, and has paused to ask next steps from this call. \textit{?pred} refers to predecessors that flow into this node within the program, and it adds context to the call to predict.  In this example it is just the constructor - "sklearn.ensemble.RandomForestClassifier". \textit{?next} shows all the calls that tend to be called on the return type of \textit{?this}, ordering by counts across the graphs in the repository. For other code assistance use case, please see~\cite{codebreaker}.

%The query locates the \textit{predict} call of \textit{RandomForestClassifier}, collects all calls that follow it and ranks them by frequency. The filter constructs ensure that only functions calls are retrieved and not their superclasses. Note that each data flow step consists of a two-edge path, {\tt \verb|sio:SIO_000230/^sio:SIO_000229|}. 




